Towards Learning to Play Piano with Dexterous Hands and Touch

The virtuoso plays the piano with passion, poetry and extraordinary technical ability. As Liszt said (a virtuoso)must call up scent and blossom, and breathe the breath of life. The strongest robots that can play a piano are based on a combination of specialized robot hands/piano and hardcoded planning algorithms. In contrast to that, in this paper, we demonstrate how an agent can learn directly from machine-readable music score to play the piano with dexterous hands on a simulated piano using reinforcement learning (RL) from scratch. We demonstrate the RL agents can not only find the correct key position but also deal with various rhythmic, volume and fingering, requirements. We achieve this by using a touch-augmented reward and a novel curriculum of tasks. We conclude by carefully studying the important aspects to enable such learning algorithms and that can potentially shed light on future research in this direction.

==> 5_discussion.tex <==
This work opens ample research opportunities for learning-based piano playing. 
Our experiments show that deep reinforcement learning can enable robot hand to play notes from scores. However, the performance would deteriorate when the task horizon length becomes longer. When end-to-end trainable agents fail to work, we combined compositional execution with the learning-based agents. Therefore, it is interesting to explore how to develop new algorithms to deal with complex long-horizon tasks. 
While our work is opening a welcoming avenue for using reinforcement learning on piano playing tasks, there are still many steps to learn to play piano with a real-world robot. 
We now briefly discuss limitations of this work and possible future works. 

The first future direction is to transfer the simulated hand and DIGIT sensor to hardware device. The domain gap between simulation and real world hardware are usually resolved by large scale domain randomization or model-based approach. Future works can learn dynamics models directly from real world data for model-based planning and/or reinforcement learning. Another possible way is to curate simulators that are perturbed in hyper-parameters for domain randomization.
%
Moreover, in this work we use reward functions that require the knowledge of instant velocity of attacked keys. Although it can be obtained from commercial electrical piano, there is not APIs designed for robotics tasks. Besides directly requesting for API, one possible way is to use tactile sensory output as surrogate for the key velocity. 
% On the robot hand side, new designs with better dexterity is required to truly enable human-level piano playing. 
%
 We also note that even the most advanced mechanical hand is not as dexterous as human hand -- this leaves a natural barrier for enabling robot hand to play music pieces wrote for pianists. We have seen efforts toward designing better hands; however, making such active hands that have similar level of dexterity to humans' remains challenging. 
 %
 In this work, we tried to minimize human inductive bias in model-free training. While it shows the high potential of an intelligent agent, in the real-world this approach would results in the equivalent of approximately 5 days to play three notes which is inefficient. We believe either learning a dynamics model or injecting more inductive bias would help the agent to learn faster. For example, imitation learning is a popular approach when sufficient expert data are available. It becomes an interesting open challenge to use existing knowledge from human pianists and human data. 
 %
 We believe these are important and promising future directions for future researchers who are interested in robot piano playing.



==> acknowledgments.tex <==
If a paper is accepted, the final camera-ready version will (and probably should) include acknowledgments. Add here thanks to reviewers who gave useful comments and to colleagues who contributed.
Different conferences have different instructions regarding funding agencies and corporate sponsors that provided financial support (sometimes in the first page, sometimes in the acknowledgments).

